Attractor-based models for sequences and pattern generation in neural circuits

Neural circuits in the brain perform a variety of essential functions, including input classification, pattern completion, and the generation of rhythms and oscillations that support processes such as breathing and locomotion. There is also substantial evidence that the brain encodes memories and processes information via sequences of neural activity. In this dissertation, we are focused on the general problem of how neural circuits encode rhythmic activity, as in central pattern generators (CPGs), as well as the encoding of sequences. Traditionally, rhythmic activity and CPGs have been modeled using coupled oscillators. Here we take a different approach, and present models for several different neural functions using threshold-linear networks. Our approach aims to unify attractor-based models (e.g., Hopfield networks) which encode static and dynamic patterns as attractors of the network. In the first half of this dissertation, we present several attractor-based models. These include: a network that can count the number of external inputs it receives; two models for locomotion, one encoding five different quadruped gaits and another encoding the orientation system of a swimming mollusk; and, finally, a model that connects the fixed point sequences with locomotion attractors to obtain a network that steps through a sequence of dynamic attractors. In the second half of the thesis, we present new theoretical results, some of which have already been published. There, we established conditions on network architectures to produce sequential attractors. Here we also include several new theorems relating the fixed points of composite networks to those of their component subnetworks, as well as a new architecture for layering networks which produces "fusion" attractors by minimizing interference between the attractors of individual layers.

==> Chapter-8.tex <==
%% !TEX root = ../Thesis.tex
%
%\chapter{Partial theoretical results, and open questions}\label{ch:open-questions}
%
%\section{Chirotope}
%
%\noindent Nov 18, 2023 - some excerpts from combinatorial geometry paper, + new s-e stuff.
%
%\subsection{G-P relations}
%Given any set of vectors $E = \{z_1,\ldots,z_m\} \subseteq \RR^{d}$, the Grassmann-Plucker (G-P) relations give us a series of identities relating determinants formed from elements of $E$. Specifically, given any $x_1,\ldots,x_{d} \in E$ and $y_1,\ldots,y_{d} \in E$,
%%
%\begin{small}
%	\begin{equation}\label{eq:G-P}
%		\det(x_1,\ldots,x_{d})\det(y_1,\ldots,y_{d}) = 
%		\sum_{\ell=1}^{d}\det(x_1,\ldots,x_{d-1},y_\ell)\det(y_1,\ldots,y_{\ell-1},x_{d},y_{\ell+1},\ldots,y_{d}).
%	\end{equation}
%\end{small}
%
%\noindent For different choices of $x_i$'s and $y_i$'s, equation~\eqref{eq:G-P} yields all possible G-P relations on $E$. Note that if $x_d = y_j$ for some $j=1,\ldots,d$, then the G-P relation is trivial.
%\medskip
%
%What do G-P relations tell us about TLNs? Recall that the rows of the $n \times (n+1)$ matrix $[-I+W \mid b]$ are the vectors
%$$h_i = (W_{i1},W_{i2},\ldots,W_{i,i-1}, -1, W_{i,i+1},\ldots,W_{in},b_i).$$
%For a TLN $(W,b)$ of dimension $n$, we are interested in the set of vectors
%$$E = E(W,b) = \{h_1,\ldots,h_n,e_1,\ldots,e_{n+1}\} \subseteq \RR^{n+1},$$ 
%corresponding to $d = n+1$. G-P relations for TLNs will relate determinants formed from these vectors, and this in turn will produce relationships among elements of the associated chirotope $\chi$. 
%
%\paragraph*{The chirotope}
%\begin{definition}
%	The {\em chirotope} $\chi = \chi_{(W,b)}$ of a TLN $(W,b)$ is the map $\chi:  E_{(W,b)}^{n+1} \to \{-1,0,1\}$, 
%	where 
%	$$\chi(v_1,\ldots,v_{n+1}) = \sgn \det(v_1,\dots,v_{n+1}),$$
%	for any $v_1,\ldots,v_{n+1} \in E_{(W,b)}$. 
%\end{definition}
%
%The reason we are interested in the chirotope $\chi$ is that it encodes the full combinatorial geometry of a TLN. In particular, $\chi$ encodes all fixed point supports in $\FP(W,b)$. 
%
%\begin{proposition}\label{prop:chirotope-FP}
%	Let $(W,b)$ be a TLN on $n$ neurons, and let $\chi: E_{(W,b)}^{n+1} \to  \{-1,0,1\}$ be its associated chirotope. Then
%	\begin{eqnarray*}
%		\quad \quad \sigma \in \FP(W,b) &\;\Leftrightarrow \; & \chi(v_1^\sigma,\ldots,v_n^\sigma,e_{i}) 
%		= \chi(v_1^\sigma,\ldots,v_n^\sigma,e_{n+1})  \text{ for all } i \in \sigma, 
%		\text{ and}\\
%		& & \chi(v_1^\sigma,\ldots,v_n^\sigma,h_{k}) 
%		= - \chi(v_1^\sigma,\ldots,v_n^\sigma,e_{n+1})   \text{ for all }  k \in [n] \setminus \sigma,\nonumber
%	\end{eqnarray*}
%	where
%	\begin{equation}\label{eq:vi^sigma}
%		v_\ell^\sigma \od \left\{\begin{array}{cc} h_i & \text{ for } \ell \in \sigma,\\
%			e_\ell & \text{ for } \ell \notin \sigma.\end{array}\right.
%	\end{equation}
%\end{proposition}
%\pagebreak
%
%\paragraph*{Some useful facts and notation}
%
%Recall that for $\sigma \subseteq [n]$, we use the notation $v_i^\sigma$
%to indicate $h_i$ or $e_i$, with 
%$v_i^\sigma = h_i$ for $i \in \sigma$ and $v_i^\sigma = e_i$ for $i \notin \sigma$ (see equation~\eqref{eq:vi^sigma}). We will also use the facts:
%
%\begin{eqnarray} \label{eq:det-facts}
%	%\det A_i^\sigma &=& \det(v_1^\sigma,\ldots,v_n^\sigma,e_i), \text{ for } i \in \sigma,\\
%	0 &=& \det(v_1^\sigma,\ldots,v_n^\sigma,e_i), \text{ for } i \in [n]\setminus \sigma, \nonumber \\
%	%\det A_\infty^\sigma &=& \det(v_1^\sigma,\ldots,v_n^\sigma,e_{n+1}), \nonumber\\
%	0 &=& \det(v_1^\sigma,\ldots,v_n^\sigma,h_i),  \text{ for } i \in \sigma, \nonumber\\
%	%\det A_i^\sigma &=& \det(v_1^\sigma,\ldots,v_n^\sigma,h_i),  \text{ for } i \notin \sigma, i \neq n+1, \nonumber\\
%	W_{ij} &=& \det(e_1,\ldots,e_{j-1},h_i,e_{j+1},\ldots,e_{n+1}), \; \text{for } i \in [n], i \neq j, \nonumber\\
%	-1 &=&  \det(e_1,\ldots,e_{i-1},h_i,e_{i+1},\ldots,e_{n+1}), \; \text{for } i \in [n], \nonumber\\
%	b_i &=& \det(e_1,\ldots,e_{n},h_i),  \text{ and} \nonumber\\
%	1 &=& \det(e_1,\ldots,e_n,e_{n+1}), \nonumber
%	%\det A_i^{\{i\}} &=& - b_i, \nonumber\\
%	%\det A_j^{\{i,j\}} &=& b_iW_{ji} + b_j \nonumber\\
%	%\det A_i^{\{i,j\}} &=& b_jW_{ij} + b_i \nonumber\\
%	%\det A_\infty^{\{i,j\}} &=& 1-W_{ij}W_{ji} \nonumber.
%\end{eqnarray}
%
%Also, recall that:
%$$\det A_j^{\{i,j\}} > 0\;\; \Leftrightarrow \;\; i \to j \quad \text{and} \quad 
%\det A_i^{\{i,j\}} > 0\;\; \Leftrightarrow \;\; j \to i.$$
%
%\noindent Finally, we will use the notation:
%\begin{equation}
%	\boxed{\quad
%		\begin{aligned}
%			\Delta_\ell^{ij} &\od  \det(e_1,\ldots,e_{\ell-1}, h_i, e_{\ell+1}, \ldots, e_n,h_j) = - \Delta_\ell^{ji}\\
%			&= W_{i\ell} \, b_j - W_{j\ell} \, b_i \quad \text{if } i,j \neq \ell.
%		\end{aligned}\quad}
%\end{equation}
%%This follows Katie's idea to insert rows $h_i$ and $h_j$ into the identity matrix $I_{n+1}$, with $\ell$ telling us where to insert $h_i$, and $h_j$ always inserted in the last row. 
%Note that for $i = j$, we always have $\Delta_\ell^{ij} = 0$. Assuming $i \neq j$, then for $\ell = i$ we obtain
%\begin{eqnarray}\label{eq:Delta-Aj}
%	\Delta_i^{ij} &= & \det(e_1,\ldots,e_{i-1}, h_i, e_{i+1}, \ldots, e_n,h_j)\\
%	&=& \det A_j^{\{i\}} = - \det A_j^{\{i,j\}} \nonumber \\
%	&=& -b_i W_{ji} - b_j, \nonumber
%\end{eqnarray}
%and for $\ell = j$ we have
%\begin{eqnarray}\label{eq:Delta-Aj}
%	\Delta_j^{ij} &= & \det(e_1,\ldots,e_{j-1}, h_i, e_{j+1}, \ldots, e_n,h_j)\\
%	&=& -\det A_i^{\{j\}} = \det A_i^{\{i,j\}} \nonumber \\
%	&=& b_jW_{ij} + b_i. \nonumber
%\end{eqnarray}
%So altogether, we get:
%$$\boxed{\;\;\Delta_\ell^{ij} = \left\{\begin{array}{cc} 
%		b_jW_{i\ell} - b_iW_{j\ell}, & \text{if } i,j \neq \ell\\
%		-b_j - b_i W_{ji}, & \text{if } i \neq j, \ell = i\\
%		-b_j W_{ij} + b_i, & \text{if } i \neq j, \ell = j\\
%		0, & \text{if } i = j.\end{array}\right.\;\;}$$
%
%\paragraph*{New $\Delta$ definition for Juliana's simply-embedded stuff}\;
%
%For any $\tau \subseteq [n]$, and $i,j,k \in [n]$, we can define:
%$$\boxed{\;\Delta_k^{ij}(\tau) \od \det(v_1^{\tau\setminus\{i,j\}},v_2^{\tau\setminus\{i,j\}},\ldots,v_{k-1}^{\tau\setminus\{i,j\}},h_i,v_{k+1}^{\tau\setminus\{i,j\}},\ldots,v_n^{\tau\setminus\{i,j\}},h_j).\;}$$
%Note that $v_i^{\tau\setminus\{i,j\}} = e_i$ and $v_j^{\tau\setminus\{i,j\}} = e_j$, so the above determinant does not repeat $h_i$ or $h_j$ terms, provided $i \neq j$, and is generically expected to be nonzero.
%For $\tau = \{i,j\}$, this new determinant reduces to:
%$$\Delta_k^{ij}(\{i,j\}) = \det(e_1,\ldots,e_{k-1},h_i,e_{k+1},\ldots,e_n,h_j) = \Delta_k^{ij}.$$
%\medskip
%
%\begin{lemma}\label{lemma:generalizeddeltas}
%	Consider a CTLN with graph $G$. Let $\tau \subseteq [n]$ be simply-embedded in $G$. Then  
%	$$\Delta_k^{ij}(\tau) = 0,$$
%	for all $i,j \in \tau$, and $k \notin \tau$.
%\end{lemma}
%
%\begin{proof}
%	If $i = j$, then $\Delta^{ij}_k = 0$ trivially ($h_i$ gets repeated). So suppose $i \neq j$.
%	WLOG, let $\tau = \{1,\ldots,i,i+1\}$, let $j = i+1,$ and $k > i+1$. Then,
%	\begin{eqnarray*}
%		\Delta_k^{ij}(\tau) &=& \det(h_1,\ldots,h_{i-1},e_i,\ldots,e_{k-1},h_i,e_{k+1},\ldots,e_n,h_j)\\
%		%&=& \left(\begin{array}{ccc} 
%		%\text{---} & h_1 & \text{---} \\
%		%\text{---} & \vdots & \text{---} \\
%		%\text{---} & h_{i-1} & \text{---}\\
%		%\text{---} & e_{i} & \text{---}\\
%		%\text{---} & \vdots & \text{---}\\
%		%\text{---} & e_{k-1} & \text{---}\\
%		%\text{---} & h_i & \text{---}\\
%		%\text{---} & e_{k+1} & \text{---}\\
%		%\text{---} & \vdots & \text{---}\\
%		%\text{---} & e_n & \text{---}\\
%		%\text{---} & h_j & \text{---}\\
%		% \end{array}\right)\\
%	&=&\det \left(\begin{array}{cccccccccccc} 
%		-1 & W_{12}  & \cdots & W_{1,i-1} & 0 & \cdots & 0 & W_{1,k} & 0 & \cdots & 0 & b_1\\
%		W_{21} & -1 & \cdots & W_{2,i-1} & 0 & \cdots & 0 & W_{2,k} & 0 & \cdots & 0 & b_2\\
%		\vdots &  &\ddots & \vdots & & \ddots &  & \vdots & & \ddots &  & \vdots\\
%		W_{i-1,1} & W_{i-1,2} & \cdots & -1 & 0 & \cdots & 0 & W_{i-1,k} & 0 & \cdots & 0 & b_{i-1}\\
%		0 & 0 & \cdots & 0 & 1 & \cdots & 0 & 0 & 0 & \cdots & 0 & 0\\
%		\vdots & \vdots &  & \vdots & &  \ddots & & \vdots & \vdots &  & \vdots & \vdots\\
%		0 & 0 & \cdots & 0 & 0 & \cdots & 1 & 0 & 0 & \cdots & 0 & 0\\
%		W_{i,1} & W_{i,2} & \cdots & W_{i,i-1} & 0 & \cdots & 0 & W_{i,k} & 0 & \cdots & 0 & b_i\\
%		0 & 0 & \cdots & 0 & 0 & \cdots & 0 & 0 & 1 & \cdots & 0 & 0\\
%		\vdots & \vdots &  & \vdots & \vdots &   & \vdots & \vdots & & \ddots &  & \vdots\\
%		0 & 0 & \cdots & 0 & 0 & \cdots & 0 & 0 & 0 & \cdots & 1 & 0\\
%		W_{j,1} & W_{j,2} & \cdots & W_{j,i-1} & 0 & \cdots & 0 & W_{j,k} & 0 & \cdots & 0 & b_j\\
%	\end{array}\right).
%\end{eqnarray*}
%Now, recall that for a CTLN we have $b_\ell = \theta$ for all $\ell \in [n]$, so the last column is of the form
%$$\theta(1,1,\ldots,1,0,\ldots,0,1,0,\ldots,0,1)^T.$$
%Furthermore, since $\tau$ is simply-embedded and $k \notin \tau$ all nonzero entries in the $k$-th column are identical and equal to $W_{i,k}$, so that this column has the form
%$$W_{i,k}(1,1,\ldots,1,0,\ldots,0,1,0,\ldots,0,1)^T.$$
%In other words, the $k$-th column is a scalar multiple of the last column, so $\Delta_k^{ij}(\tau) = 0$.
%\end{proof}
%
%\begin{lemma}\label{lemma:vanishingdets}
%Consider a CTLN with graph $G$. Let $\tau \subseteq [n]$ be simply-embedded in $G$. Any chirotope element whose only $h_i$ elements come from $\tau$ ($i\in\tau$), and does not contain $e_p,e_q$ for some $p,q\notin\tau$, will vanish.
%\end{lemma}
%
%\begin{proof}
%Let $\sigma = \{1,...,k\} \subseteq \tau$. It suffices to prove:
%\begin{equation}\label{eq:vanishingdet}
%	\det(h_1,\dots,h_k,e_{s_{1}},\dots,\widehat{e_p},\dots,\widehat{e_q}\dots,e_{s_{n+1-k}}) = 0,
%\end{equation} as other determinants satisfying the conditions in the theorem are either permutations or index relabelings of the LHS of (\ref{eq:vanishingdet}). Let $\rho = \tau \setminus \sigma = \{k+1,\dots,l\}$, and $[n]\setminus\tau = \{l+1,\dots,p,\dots,q,\dots,n\}$ then
%\begin{align*}
%	&\det(h_1,\dots,h_k,e_{s_{1}},\dots,\widehat{e_p},\dots,\widehat{e_q}\dots,e_{s_{n+1-k}}) \\
%	= &\det\left(\begin{array}{c|c|ccccccc|c}
%		& & W_{1,l+1} & & W_{1,p} & &W_{1,q}& &W_{1,n}&\theta\\
%		\sigma \rightarrow \sigma & \rho \rightarrow \sigma &\vdots& \cdots & \vdots & \cdots &\vdots& \cdots &\vdots&\vdots\\
%		& & W_{k,l+1} & & W_{k,p} & &W_{k,q}& &W_{k,n}&\theta\\
%		\hline
%		& &  & & 0 & &0& & &\\
%		*&*&*& \cdots & \vdots & \cdots &\vdots& \cdots &*&*\\
%		& &   & & 0 & &0& & &
%	\end{array}\right)
%\end{align*}
%But since $\tau$ is simply-embedded, $W_{i,j} = W_{j}$ for all $i \in \tau$ and $j \notin\tau$ and therefore columns $p$ and $q$ are linearly dependent:
%\begin{align*}
%	&\det\left(\begin{array}{c|c|ccccccc|c}
%		& & W_{l+1} & & W_{p} & &W_{q}& &W_{n}&\theta\\
%		\sigma \rightarrow \sigma & \rho \rightarrow \sigma &\vdots& \cdots & \vdots & \cdots &\vdots& \cdots &\vdots&\vdots\\
%		& & W_{l+1} & & W_{p} & &W_{q}& &W_{n}&\theta\\
%		\hline
%		& &  & & 0 & &0& & &\\
%		*&*&*& \cdots & \vdots & \cdots &\vdots& \cdots &*&*\\
%		& &   & & 0 & &0& & &
%	\end{array}\right) = 0.
%\end{align*}
%Note however that the other columns may or may not be linearly dependent, as the * indicates the possible presence of a $1$, so it is indeed necessary to have $e_p$ and $e_q$ not appear in the determinant. Also, note that the proof still holds if $q=n+1$.
%\end{proof}
%
%Lemma \ref{lemma:generalizeddeltas} now follows from Lemma \ref{lemma:vanishingdets}:
%\begin{align*}
%\Delta_k^{ij}(\tau) = &\det(h_1,\ldots,h_{i-1},e_i,e_{i+1},e_{i+2}\ldots,e_{k-1},h_i,e_{k+1},\ldots,e_n,h_j)\\
%= \pm &\det(h_1,\ldots,h_{i-1},h_i,h_{j},e_{i+2},\ldots,e_{k-1},e_i,e_{k+1},\ldots,e_n,e_{i+1})\\
%= \pm &\det(h_1,\ldots,h_{j=i+1},e_i,e_{i+1},e_{i+2}\ldots,e_{k-1},e_{k+1},\ldots,e_n).
%\end{align*}
%It is clear from the last determinant that $e_k$ and $e_{n+1}$ are missing, with $k,n+1 \notin \tau = \{1,\ldots,i,i+1\}$. In this case, $\sigma = \tau$ in the proof above. Note that the indices above give a total of $n+1$ elements: $1,\dots,k-1,k+1,\dots,n$ with an extra $i,i+1$ for a total of $n-1+2 = n+1$ elements.
%
%\begin{lemma}\label{lemma:vanishingdetsv2} 
%Let $\tau \subseteq [n]$ and suppose one of the following holds:
%\begin{enumerate}
%	\item There exist $p,q \in [n] \setminus \tau$, $(p \neq q)$ such that $\tau$ is simply-embedded in $\tau \cup \{p,q\}$. That is, $W_{i,p} = W_{j,p}$  and $W_{i,q} = W_{j,q}$ for all $i,j \in \tau$. (Assume no restrictions on $b$).
%	\item There exists $p \in [n] \setminus \tau$ such that $\tau$ is simply-embedded in $\tau \cup \{p\}$, $q = n+1$, and $b_i = \theta$ for all $i \in \tau$ (it can be anything outside of $\tau$).
%\end{enumerate}
%Then, any chirotope determinant whose only $h_i$ elements come from $\tau$ (i.e. $i \in \tau$), and does not contain $e_p$ or $e_q$, will vanish.
%\end{lemma}
%
%\begin{proof}
%Let $\sigma = \{1,...,k\} \subseteq \tau$. It suffices to prove:
%\begin{equation}\label{eq:vanishingdetv2}
%	\det(h_1,\dots,h_k,e_{s_{1}},\dots,\widehat{e_p},\dots,\widehat{e_q}\dots,e_{s_{n+1-k}}) = 0,
%\end{equation} as other determinants satisfying the conditions in the theorem are either permutations or index relabelings of the LHS of (\ref{eq:vanishingdetv2}). 
%First, suppose (i) holds. Let $\rho = \tau \setminus \sigma = \{k+1,\dots,l\}$, and $[n]\setminus\tau = \{l+1,\dots,p,\dots,q,\dots,n\}$, then
%\begin{align*}
%	&\det(h_1,\dots,h_k,e_{s_{1}},\dots,\widehat{e_p},\dots,\widehat{e_q}\dots,e_{s_{n+1-k}}) \\
%	= &\det\left(\begin{array}{c|c|ccccccc|c}
%		& & W_{1,l+1} & & W_{1,p} & &W_{1,q}& &W_{1,n}&b_1\\
%		\sigma \rightarrow \sigma & \rho \rightarrow \sigma &\vdots& \cdots & \vdots & \cdots &\vdots& \cdots &\vdots&\vdots\\
%		& & W_{k,l+1} & & W_{k,p} & &W_{k,q}& &W_{k,n}&b_n\\
%		\hline
%		& &  & & 0 & &0& & &\\
%		*&*&*& \cdots & \vdots & \cdots &\vdots& \cdots &*&*\\
%		& &   & & 0 & &0& & &
%	\end{array}\right),
%\end{align*} where the $*$ are blocks of mostly zeros and some ones, coming from the $e_{s_i}$ rows.
%Now, since $\tau$ is simply-embedded in $\tau \cup \{p,q\}$, it follows that columns $p$ and $q$ are linearly dependent and thus the determinant vanishes.
%
%For (ii), let $\rho = \tau \setminus \sigma = \{k+1,\dots,l\}$, and $[n]\setminus\tau = \{l+1,\dots,p,\dots,n\}$. Then the determinant looks like
%\begin{align*}
%	&\det(h_1,\dots,h_k,e_{s_{1}},\dots,\widehat{e_p},\dots,\widehat{e_{n+1}}\dots,e_{s_{n+1-k}}) \\
%	= &\det\left(\begin{array}{c|c|ccccc|c}
%		& & W_{1,l+1} & & W_{1,p} & &W_{1,n}&\theta\\
%		\sigma \rightarrow \sigma & \rho \rightarrow \sigma &\vdots& \cdots & \vdots & \cdots &\vdots&\vdots\\
%		& & W_{k,l+1} & & W_{k,p} & &W_{k,n}&\theta\\
%		\hline
%		& &  & & 0 & & &0\\
%		*&*&*& \cdots & \vdots & \cdots &*&\vdots\\
%		& &   & & 0 & & &0
%	\end{array}\right)
%\end{align*} and so in this case columns $p$ and $n+1$ are linearly dependent too, and the determinant vanishes.
%\end{proof}

==> UserDefinedCommands.tex <==

% Define the \acro command.
\makeatletter
\newif\ifFirstPar       \FirstParfalse
\def\smc{\sc}
\def\ninepoint{\small}
\DeclareRobustCommand\SMC{%
  \ifx\@currsize\normalsize\small\else
   \ifx\@currsize\small\footnotesize\else
    \ifx\@currsize\footnotesize\scriptsize\else
     \ifx\@currsize\large\normalsize\else
      \ifx\@currsize\Large\large\else
       \ifx\@currsize\LARGE\Large\else
        \ifx\@currsize\scriptsize\tiny\else
         \ifx\@currsize\tiny\tiny\else
          \ifx\@currsize\huge\LARGE\else
           \ifx\@currsize\Huge\huge\else
            \small\SMC@unknown@warning
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}
\newcommand\SMC@unknown@warning{\TBWarning{\string\SMC: unrecognised
    text font size command -- using \string\small}}
\newcommand\textSMC[1]{{\SMC #1}}
\newcommand\acro[1]{\textSMC{#1}\@}

\makeatother

% command for vectors
\newcommand{\bv}[1]{\ensuremath{\vec{#1}}}
% command for unit vectors
\newcommand{\uv}[2][blank]{%
\ifthenelse{\equal{#1}{blank}}%
{\ensuremath{\hat{u}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{.}}%
{\ensuremath{\dot{\hat{u}}_{#2}}}%
{}%
%
\ifthenelse{\equal{#1}{'}}%
{\ensuremath{\hat{u}'_{#2}}}%
{}%
}
\newcommand{\ui}{\ensuremath{\hat{\imath}}}
\newcommand{\uj}{\ensuremath{\hat{\jmath}}}
\newcommand{\uk}{\ensuremath{\hat{k}}}


%%my commands start here jla

\def\mybullet{{$\circ\,\,$}}
\newcommand{\od}{\stackrel{\mbox {\tiny {def}}}{=}}
\newcommand{\Fix}{{\operatorname{Fix}}}
\def\CC{\mathbb{C}}
\def\eigs{\operatorname{eigenvals}}
\def\d{\mathrm{d}}
\def\mybullet{{$\circ\,\,$}}
\def\RR{\mathbb{R}}
\def\QQ{\mathbb{Q}}
\def\ZZ{\mathbb{Z}}
\def\RN{{\mathbb{R}^N}}
\def\RNplus{{\mathbb{R}^N_{\geq 0}}}
\def\U{\mathcal{U}}
\def\J{\mathcal{J}}
\def\for{\mathrm{for}}
\def\where{\mathrm{where}}
\def\Spec{\mathrm{Spec}}
\def\geom{\mathrm{geom}}
\def\S{{\mathcal{S}}}
\def\C{\mathcal{C}}
\def\P{\mathcal{P}}
\def\Fix#1{{\operatorname{Fix}_{{#1}}}}
\def\mtx#1#2#3#4{\left(\begin{array}{cc} #1 & #2 \\ #3 & #4 \end{array} \right)} 
\def\syseq#1#2#3#4{\left\{ \begin{array}{ccc} #1 &=& #2 \\ #3 &=& #4 \end{array} \right.} 
\def\tf#1{{\left[#1\right]_+}}
\def\lm#1{\lambda_{\operatorname{max}}(#1)}
\def\One#1{{1_{#1}}}
\def\mybullet{{$\circ\,\,$}}
\def\RR{\mathbb{R}}
\def\RN{{\mathbb{R}^N}}
\def\RNplus{{\mathbb{R}^N_{\geq 0}}}
\def\U{\mathcal{U}}
\def\M{\mathcal{M}}
\def\for{\mathrm{for}}
\def\where{\mathrm{where}}
\def\Spec{\mathrm{Spec}}
\def\geom{\mathrm{geom}}
\def\tr{\operatorname{tr}}
\def\det{\operatorname{det}}
\def\S{{\mathcal{S}}}
\def\C{\mathcal{C}}
\def\P{\mathcal{P}}
\def\F{\mathcal{F}}
\def\G{\mathcal{G}}
\def\Ncells{\mathrm{N}_{\mathrm{cells}}}
\def\vsp{\vspace{-.25cm}}
\def\wtilde#1{\widetilde{#1}}
\def\widetildeG{\wtilde{G}}
\def\what#1{\widehat{#1}}
\def\max{\mathrm{max}}
\def\norm#1{\left\|#1\right\|}
\def\supp{\operatorname{supp}}
\def\CM{\mathcal{C}}
\renewcommand{\v}{\mathbf}
\def\od{\stackrel{\mathrm{def}}{=}}
\def\ml{\mathrm{ML}}
\def\stab{\operatorname{stab}}
\def\negsp{\hspace{-.075in}}
\def\K{\mathcal{K}}
\def\O{\mathcal{O}}
\def\nn{ \{1,...,n\}}
\def\supp{\operatorname{supp}}
\def\CF{\operatorname{CF}}
\def\cm{\mathrm{cm}}
\def\CM#1{\left|\dfrac{\mathrm{cm}(#1)}{\det(#1)}\right|}
\def\CMinv#1{\left|\dfrac{\det(#1)}{\mathrm{cm}(#1)}\right|}
\def\conv#1{\operatorname{conv}\{#1\}}
\def\diag{\operatorname{diag}}
\def\sgn{\operatorname{sgn}}
\def\FP{\operatorname{FP}}
\def\type{\operatorname{type}}
\def\idx{\operatorname{idx}}
\def\Wtil{\widetilde{W}}
\def\eig{\operatorname{eig}}
\def\one{\mathbf{1}}
\def\Ghat{\widehat G}
\newcommand{\rotvert}{\rotatebox[origin=c]{90}{$\vert$}}


%%%%%%%%%%%%%%%%%%%%%% theorems, operators, ... %%%%%%%%%%%%%%%%%%%%%%%%


% comments defns
\definecolor{cherry}{rgb}{0.9,.1,.2}
\def\cherry#1{\textcolor{cherry}{#1}}
\def\carina#1{{\tt [#1]}}
\def\katie#1{\cherry{\tt [#1]}}
\def\caitlyn#1{\cherry{\tt [#1]}}
\definecolor{turquoise}{rgb}{.188, .835, .784}
\def\turquoise#1{\textcolor{turquoise}{#1}}
\def\juliana#1{\turquoise{\tt [#1]}}

%quadruped gaits colors
\definecolor{leg1_color}{rgb}{0.7922,    0.5490,    0.1686}
\definecolor{leg2_color}{rgb}{0.7961,    0.1294,    0.1569}
\definecolor{leg3_color}{rgb}{0.0706,    0.5020,    0.6980}
\definecolor{leg4_color}{rgb}{0.1647,    0.6000,    0.2784}
\definecolor{bound_aux_color}{rgb}{0.9451,    0.3765,    0.4157}
\definecolor{pace_aux_color}{rgb}{0.4980,    0.7725,    0.9294}
\definecolor{trot_aux_color}{rgb}{0.4118,    0.7569,    0.5255}
\definecolor{walk_aux_color}{rgb}{1.0000,    0.8118,    0.2941}
\definecolor{pronk_aux_color}{rgb}{0.9373,    0.3412,    0.1451}

\newcommand\legone[1]{\textcolor{leg1_color}{\textbf{#1}}}
\newcommand\legtwo[1]{\textcolor{leg2_color}{\textbf{#1}}}
\newcommand\legthree[1]{\textcolor{leg3_color}{\textbf{#1}}}
\newcommand\legfour[1]{\textcolor{leg4_color}{\textbf{#1}}}

\newcommand\boundaux[1]{\textcolor{bound_aux_color}{#1}}
\newcommand\paceaux[1]{\textcolor{pace_aux_color}{#1}}
\newcommand\trotaux[1]{\textcolor{trot_aux_color}{#1}}
\newcommand\walkaux[1]{\textcolor{walk_aux_color}{#1}}
\newcommand\pronkaux[1]{\textcolor{pronk_aux_color}{#1}}

%theorems
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{facts}[theorem]{Facts}
%\newtheorem*{theoremA}{Theorem A}
%\newtheorem*{theoremB}{Theorem B}
%\newtheorem*{theoremC}{Theorem C}
%\newtheorem*{theoremD}{Theorem D}
%\newtheorem*{theoremE}{Theorem E}
%\newtheorem*{theoremF}{Theorem F}
%\newtheorem*{theoremG}{Theorem G}
%\newtheorem*{theoremH}{Theorem H}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{definitions}[theorem]{Definitions}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{question}[theorem]{Question}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem*{claim}{Claim}
\newtheorem{answer}[theorem]{Answer}
\newtheorem{defn}{Definition}
\newtheorem{myquestion}{Question}
\newtheorem{myanswer}{Answer}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{rules}{Rule}

